Scalable Estimation for Structured Additive Distributional Regression Through Variational Inference

Structured additive distributional regression models offer a versatile framework for estimating complete conditional distributions by relating all parameters of a parametric distribution to covariates. Although these models efficiently leverage information in vast and intricate data sets, they often result in highly-parameterized models with many unknowns. Standard estimation methods, like Bayesian approaches based on Markov chain Monte Carlo methods, face challenges in estimating these models due to their complexity and costliness. To overcome these issues, we suggest a fast and scalable alternative based on variational inference. Our approach combines a parsimonious parametric approximation for the posteriors of regression coefficients, with the exact conditional posterior for hyperparameters. For optimization, we use a stochastic gradient ascent method combined with an efficient strategy to reduce the variance of estimators. We provide theoretical properties and investigate global and local annealing to enhance robustness, particularly against data outliers. Our implementation is very general, allowing us to include various functional effects like penalized splines or complex tensor product interactions. In a simulation study, we demonstrate the efficacy of our approach in terms of accuracy and computation time. Lastly, we present two real examples illustrating the modeling of infectious COVID-19 outbreaks and outlier detection in brain activity.

==> defs_letter.tex <==
\setlength{\topmargin}{-0.75in}
\setlength{\textheight}{9.5in}
\setlength{\oddsidemargin}{0pt}
%\textwidth 440pt 
\setlength{\textwidth}{6.5in}%width for US letterhead paper 
\parskip 0pt
\newcounter{num}
\newcommand{\utilde}[1]{\mathrel{\mathop{#1}\limits_{\displaystyle \widetilde{}}}}
%\def\baselinestretch{1.22}
\def\theequation{\thesection.\arabic{equation}}  
\def\abstract{\if@twocolumn
\section*{Abstract}
\else \normalsize 
\begin{center}
{\bf Summary\vspace{-.5em}\vspace{0pt}} 
\end{center}
\quotation 
\fi}
\def\endabstract{\if@twocolumn\else\endquotation\fi}
\newcommand{\bfy}{\mbox{{\bf y}}}
\newcommand{\bfw}{\mbox{\boldmath $w$}}
\newcommand{\bfs}{\mbox{\boldmath $s$}}
\newcommand{\bfg}{\mbox{\boldmath $g$}}
\newcommand{\bfu}{\mbox{\boldmath $u$}}
\newcommand{\bfv}{\mbox{\boldmath $v$}}
\newcommand{\bfx}{\mbox{\boldmath $x$}}
\newcommand{\bfzero}{\mbox{{\bf 0}}}
\newcommand{\bfalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bff}{\mbox{{\bf f}}}
\newcommand{\bfb}{\mbox{{\bf b}}}
\newcommand{\bfone}{\mbox{{\bf 1}}}
\newcommand{\bfZ}{\mbox{\boldmath $Z$}}
\newcommand{\bfe}{\mbox{{\bf e}}}
\newcommand{\bfr}{\mbox{{\bf r}}}
\newcommand{\bfz}{\mbox{{\bf z}}}
\newcommand{\told}{\mbox{{\tiny old}}}
\newcommand{\tnew}{\mbox{{\tiny new}}}
\newcommand{\gammanew}{\mbox{$\gamma^{\tnew}$}}
\newcommand{\gammajnew}{\mbox{$\gamma^{\tnew}_j$}}
\newcommand{\gammaold}{\mbox{$\gamma^{\told}$}}
\newcommand{\gammajold}{\mbox{$\gamma^{\told}_j$}}
\newcommand{\zetan}{\mbox{$\zeta^{\tnew}$}}
\newcommand{\zetao}{\mbox{$\zeta^{\told}$}}
\newcommand{\phin}{\mbox{$\phi^{\tnew}$}}
\newcommand{\phio}{\mbox{$\phi^{\told}$}}
\newcommand{\phitn}{\mbox{$\tilde \phi^{\tnew}$}}
\newcommand{\phito}{\mbox{$\tilde \phi^{\told}$}}
\newcommand{\bfJ}{\mbox{\boldmath $J$}}
\newcommand{\bfpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bfepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bfomega}{\mbox{\boldmath $\omega$}}
\newcommand{\bfkappa}{\mbox{\boldmath $\kappa$}}
\newcommand{\bftheta}{\mbox{\boldmath $\theta$}}
\newcommand{\half}{\mathop{\frac{1}{2}}}
\newcommand{\var}{\mathop{\rm var}} 
\newcommand{\Exp}{\mathop{\rm E}}
\newcommand{\cov}{\mathop{\rm cov}}
\newcommand{\corr}{\mathop{\rm corr}}
\newcommand{\load}{\mbox{LOAD}}
%\newcommand{\temp}{\mbox{TEMP}}
\newcommand{\hmd}{\mbox{HMD}}
\newcommand{\toy}{\mbox{TOY}}
\newcommand{\dum}{\mbox{DUM}}
\newcommand{\rowspace}{\mathop{\rm row~space}}
\makeatletter
\newcommand{\myappendix}[1]{
%	\renewcommand{\thesection}{{\bf Appendix}~{\bf \Alph{section}}}
%	\section{#1}
	\setcounter{section}{1}
%	\renewcommand{\thesection}{\Alph{section}}} 
        \renewcommand{\thesection}{A\arabic{section}}}

\newcommand{\fah}[1]{
	\vspace{-0.2in}\nopagebreak
	\begin{center}
		{\sf -----#1-----}
	\end{center}\nopagebreak
	\vspace{-0.1in}}

